A Geometria da Regress\~ao Linear

We present a geometrical interpretation of linear regression based on vectors in n dimensions (n the number of data points). This is to be used as a didactic tool for teachers when presenting that topic.

==> figura1.tex <==
\beginpicture
\linethickness=1pt
\setcoordinatesystem units < 0.7cm, 0.7cm>
\setplotarea x from -3.5 to  3, y from -3 to  4
\axis left shiftedto x=0  / 
\axis bottom shiftedto y=0  / 
\linethickness=0.4pt
\setplotsymbol({\Large .})
\put {$\bullet$} at -3 -.4  
\put {$\bullet$} at -2.5  1  
\put {$\bullet$} at -1.5  1  
\put {$\bullet$} at -.5  2  
\put {$\bullet$} at  .5  3  
\put {$\bullet$} at  1  2.5  
\put {$\circ$} at -1  1.5 
\put {$\bullet$} at -2 -1.9  
\put {$\bullet$} at -1.5 -.5  
\put {$\bullet$} at -.5 -.5  
\put {$\bullet$} at  .5  .5  
\put {$\bullet$} at  1.5  1.5  
\put {$\bullet$} at  2  1  
\put {$\circ$} at  0  0  
\setplotsymbol({\tiny .})
\setplotsymbol  ({\large .})
\plot  -3.5 -.495     2  3.85 /  
\plot  -3.5 -2.765     3  2.37 /  
\setplotsymbol  ({\tiny .})
\arrow < 2mm>  [ .2679492, 1.154701] from  -2.16718  2.27812 to -1.16641  1.61094
\arrow < 2mm>  [ .2679492, 1.154701] from   1.217157 -1.217157 to  .1414214 -.1414214
\put {$(\bar x,\bar y)$} at -2.7  2.7
\put {$(\bar{\tilde{x}},\bar{\tilde{y}})$} at  1.7 -1.7
\put {$y=ax+b$} at  2  4.15
\put {$\tilde{y}=a\tilde{x}$} at  3  2.57
\endpicture

